SnakeGAN: A Universal Vocoder Leveraging DDSP Prior Knowledge and Periodic Inductive Bias

Generative adversarial network (GAN)-based neural vocoders have been widely used in audio synthesis tasks due to their high generation quality, efficient inference, and small computation footprint. However, it is still challenging to train a universal vocoder which can generalize well to out-of-domain (OOD) scenarios, such as unseen speaking styles, non-speech vocalization, singing, and musical pieces. In this work, we propose SnakeGAN, a GAN-based universal vocoder, which can synthesize high-fidelity audio in various OOD scenarios. SnakeGAN takes a coarse-grained signal generated by a differentiable digital signal processing (DDSP) model as prior knowledge, aiming at recovering high-fidelity waveform from a Mel-spectrogram. We introduce periodic nonlinearities through the Snake activation function and anti-aliased representation into the generator, which further brings the desired inductive bias for audio synthesis and significantly improves the extrapolation capacity for universal vocoding in unseen scenarios. To validate the effectiveness of our proposed method, we train SnakeGAN with only speech data and evaluate its performance for various OOD distributions with both subjective and objective metrics. Experimental results show that SnakeGAN significantly outperforms the compared approaches and can generate high-fidelity audio samples including unseen speakers with unseen styles, singing voices, instrumental pieces, and nonverbal vocalization.

==> img/RS_model.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{images/RS_model.png}
  \caption{Recognition-synthesis based model architecture.$T_s$ means the number of frames in time axis.}
  \label{fig:Rec_Syn_model}
\end{figure}
%22

==> img/abx.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{images/ABX.png}
  \caption{ABX test for similarity, NP means no preference.}
  \label{fig:ABX}
\end{figure}

==> img/proposed.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{images/Proposed.png}
  \caption{The proposed acoustic model, FFT Block is the feed forward transformer structure proposed in \cite{ren2019fastspeech}. (a). The overall structure. (b). The Embedding Discriminator distinguishes whether an input content embedding is extracted from external corpora. (c) The Conversion Discriminator distinguishes whether an input Mel has been converted by the acoustic model. (d) The Real/Fake Discriminator distinguishes whether an input Mel is reconstructed by the acoustic model.}
  \label{fig:proposed_img}
\end{figure*}

==> img/visual_contentemb.tex <==
\begin{figure}[t]
\begin{minipage}[b]{1.0\linewidth}
  \centering
% \centerline{\epsfig{figure=image1.ps,width=8.5cm}}
  % \vspace{1.5cm}
  \includegraphics[width=1.0\linewidth]{images/visual_a.png}
  \centerline{(a) Without $\mathcal{L}_{sim}$}\medskip
\end{minipage}
%
\begin{minipage}[b]{1.0\linewidth}
  \centering
% \centerline{\epsfig{figure=image1.ps,width=8.5cm}}
  % \vspace{1.5cm}
  \includegraphics[width=1.0\linewidth]{images/visual_b.png}
  \centerline{(b) With $\mathcal{L}_{sim}$ }\medskip
\end{minipage}
%
\caption{T-SNE visualization in content embedding extracted from different SSL representations. The scatters in different colors belong to different speakers.}
\label{fig:visual_contemb}
\end{figure}

==> table/obj_exp.tex <==



\begin{table}[h]
    % \vspace{-1.0 em}
    \centering
    \small
	\caption{
	%The  
	% MCD, Energy and F0 RMSE 
 Objective experiments calculated between the waveforms generated by different systems.
 	Energy 
 	%RMSE 
 	and F0 RMSEs were calculated between \textbf{source} and \textbf{converted} waveform while MCD and COS-SIM was calculated between %parallel
 	\textbf{target} and \textbf{converted} waveform. 
  % COS-SIM is calculated between speaker embedding extracted from converted and target Mel.
	}
	\label{tab:Objct}
	% \centering
        % \resizebox{\linewidth}{!}{
	\begin{tabular}{lcccc}
	\toprule
	\small{Model} &\small{MCD} &\small{COS-SIM} &\small{Energy RMSE} &\small{F0 RMSE}\\
        % \midrule
        \hline

        \small{Hubert Soft} &\textbf{5.600} &\textbf{0.889} &0.156 &0.251 \\
        \small{w/o $\mathcal{L}_{r/f}$} &5.709 &0.877 &0.176 &0.296\\
        \small{w/o $\mathcal{L}_{e}$} &5.717 &0.880 &0.160 &0.294\\
	\small{w/o $\mathcal{L}_{sim}$} &5.813 &0.833 &0.119  &0.246 \\ 
        %\small{w/$\mathcal{L}_{sim}$} &\textbf{5.600} &\textbf{0.889} &0.156 &0.251 \\
        
        % \cline{1-5}
        \hline
        \small{Hubert Raw} &\textbf{5.846} &\textbf{0.882} &0.152 &0.211 \\
        \small{w/o $\mathcal{L}_{r/f}$} &5.978 &0.880 &0.144 &0.371\\
        \small{w/o $\mathcal{L}_{e}$} &5.943 &0.883 &0.185 &0.330\\
        \small{w/o $\mathcal{L}_{sim}$} &5.970 &0.746  &0.103 &0.212 \\ 
        % \cline{1-5}
        \hline
        \small{ContentVec} &5.739 &0.880 &0.159 &0.277 \\
        \small{w/o $\mathcal{L}_{r/f}$} &\textbf{5.664} &\textbf{0.891} &0.208 &0.338\\
        \small{w/o $\mathcal{L}_{e}$} &5.784 &0.883 &0.174 &0.311\\
        \small{w/o $\mathcal{L}_{sim}$} &5.797 &0.868  &0.136 &0.236 \\ 
        % \cline{1-5}
        \hline
        \small{CTC BNFs} &5.476 &0.873 &0.173 &0.272 \\ 
	\bottomrule
        \end{tabular}
        % }
\end{table}


==> table/sub_exp.tex <==




\begin{table}[ht]
    % \vspace{-1.0 em}
    \centering
    \small
	\caption{
	The MOS with 95\% confidence intervals in Naturalness and Similarity.
	}
	\label{tab:subj}
	\begin{tabular}{lcc}
		\toprule
		 &\small{Naturalness} 
		 &\small{Similarity} \\
		
        % \midrule
        \hline
	\small{Hubert Soft} 
	&4.183(±0.193)
	&3.985(±0.212)  \\
		
        \small{w/o $\mathcal{L}_{sim}$ (Baseline)} 
        &4.267(±0.183)
        &3.584(±0.185)\\ 
        % \cline{1-3}
        \hline
        \small{Hubert Raw} 
        &4.366(±0.249)
        &4.142(±0.278)\\
        \small{w/o $\mathcal{L}_{sim}$ (Baseline)} 
        &4.200(±0.316)
        &3.114(±0.216) \\ 
        % \cline{1-3}
        \hline
        \small{ContentVec} 
        &3.771(±0.289)
        &4.030(±0.261)\\ 
        \small{w/o $\mathcal{L}_{sim}$ (Baseline)} 
        &4.086(±0.304)
        &3.550(±0.260)\\ 
        % \bottomrule
        \hline
        \small{CTC BNFs} 
        &3.460(±0.235)
        &4.153(±0.197)\\ 
        
	\bottomrule
	\end{tabular}
\end{table}
